What makes people bond?: A study on social interactions and common life points on Facebook

In this paper we aim at understanding if and how, by analysing people's profile and historical data (such as data available on Facebook profiles and interactions, or collected explicitly) we can motivate two persons to interact and eventually create long-term bonds. We do this by exploring the relationship between connectedness, social interactions and common life points on Facebook. The results are of particular importance for the development of technology that aims at reducing social isolation for people with less chances to interact, such as older adults.

==> background.tex <==
% !TEX root = main.tex

\section{Background}
visits and surveys

\subsection{Visits to nursing homes}
describe methods,
-not many friendships are developed in nursing homes

\subsection{surveys} 
lack of topics of conversation
- refer paper in persuasive, salzburg
- use charts from workshop


